Generic and Trend-aware Curriculum Learning for Relation Extraction in Graph Neural Networks

We present a generic and trend-aware curriculum learning approach for graph neural networks. It extends existing approaches by incorporating sample-level loss trends to better discriminate easier from harder samples and schedule them for training. The model effectively integrates textual and structural information for relation extraction in text graphs. Experimental results show that the model provides robust estimations of sample difficulty and shows sizable improvement over the state-of-the-art approaches across several datasets.

==> sections/additional_results.tex <==
\begin{table*}[t]\small
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
 {\bf Additional Features} & {\bf Initial Embeddings}  & \multicolumn{3}{c}{{\bf GDPR}} & \multicolumn{3}{|c|}{{\bf PGR}}\\ \hline
 & & {\bf Precision} & {\bf Recall} & {\bf F1} & {\bf Precision} & {\bf Recall} & {\bf F1} \\ \hline
 \multirow{3}{*}{No} & Random & 32.09 & 41.17 & 36.07 & 81.70 &89.33  &85.35 \\
 & BioBERT &46.42 &02.06 & 03.95& 80.82 & 78.66 & 79.72\\
 & Doc2Vec  &72.93 & 35.00 & 47.00   & 83.54 & 88.00 & 85.71 \\ \hline
 \multirow{3}{*}{Yes} & Random & 64.71& \textbf{72.01} & 68.17 & 82.71 & \textbf{89.33} &85.89 \\
 & BioBERT & 73.99 & 52.46 &  61.39 & 86.95 & 80.00 & 83.33\\
 & Doc2Vec & \textbf{76.86} & 70.27& \textbf{73.42} & \textbf{86.84} & 88.00 & \textbf{87.41}\\ \hline
\end{tabular}
\caption{Effect of initial node embeddings and additional textual features using graph neural network on predicting causality between gene-disease/phenotype.}
%\nidhi{Here, no additional features with initial embeddings will be considered as GrapgSAGE?? }
%\hadi{yes and no, I think it's fine to keep this table as it is; it's important to know your model's performance with and w/o additional features.}
\label{ablation_study}
\end{table*}


\begin{table*}[!h]\small
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|} \hline
    {\bf Model} &  \multicolumn{3}{c}{{\bf GDPR} (Gene-Disease)} & \multicolumn{3}{|c|}{{\bf GDPR} (Gene-Phenotype)} & \multicolumn{3}{|c|}{{\bf PGR} (Gene-Phenotype)} \\ \hline
    & {\bf Precision} & {\bf Recall} & {\bf F1} & {\bf Precision} & {\bf Recall} & {\bf F1} & {\bf Precision} & {\bf Recall} & {\bf F1} \\ \hline
    %{\bf All ones} & 50.00 & 100.00 & 66.66 & -- & -- & --\\ \hline
    {\bf Co-occurrence} & 50.00 & 100.00 & 66.66 & 50.00 & 100.00 & 66.66 & 47.46 & 100.00 & 64.37 
     \\ \hline
    {\bf Relevance score} & 83.57 & 58.98 & 69.09 &52.06  & 06.48 & 11.53 & 72.73 & 21.33  & 32.99 
      \\ \hline
    %{\bf BoLSTM} & -- & -- & --& & & \\ \hline
    {\bf BioBERT} & 63.87 & 59.30 &61.50 & 76.86 & 73.87 & 75.33 & 81.82  & 72.00 &  76.60
    \\ \hline
    {\bf GraphSAGE+Doc2Vec} &72.93 & 35.00 & 47.00 & 81.84 & 84.71 & 83.25  & 83.54 & 88.00 &  85.71
     \\\hline
    \hline
    {\bf \SYSNAME} & 76.86 & 70.27 & {\bf 73.42$^$*} & 82.67 & 86.10 & {\bf84.35$^$*} & 86.84 & 88.00 & {\bf 87.41$^$*} 
      \\ \hline
    \end{tabular}
    \caption{Performance of different models on relation prediction for GDPR and PGR dataset. For a fair comparison for bench-marking, we evaluated gene-phenotype relations present in the GDPR graph using existing PGR dataset as it has been used before and gene-phenotypes pairs present in PGR  overlaps  with GDPR. 
    %\hadi{swap columns 2\&3}
    %\nidhi{\SYSNAME{} significantly outperforms BioBERT with p-value < 1\% and GraphSAGE with p-value <2\%.}
    %\hadi{need to include All Ones results for PGR.} \nidhi{that  would be same as Co-occurrence score, as that considers all the extracted pairs as positive}\hadi{how about removing all ones then and only including co-occurrence? for GDPR all will be labeled as non-causal, so p would be .5 and recall 1.}
    }
    %\hadi{should we call {\bf \SYSNAME{} w/o add. features} GraphSage and use it as a baseline to illustrate we have good baselines?}
    %\hadi{Reviewers may ask why don't you report results on GDPR (Gene-Phenotype)... perhaps we could say we resort to PGR for that task..}
    %\nidhi{(p-value < 1 \% for BioBERT, p < 2 \% for GraphSAGE) } 
    \label{performance}
\end{table*}

==> sections/data.tex <==
% \section{GDPR Dataset}


% \begin{table}[]
%     \centering
%     \begin{tabular}{|p{4cm}|l|}
%         \hline
%          \# of Genes &  4274\\
%          \hline
%          Number of Disease Series & 472\\
%          \hline
%          Number of Disease & 6143\\
%          \hline
%          Number of Total Nodes & 10889\\
%          \hline
%          Number of edges & 10196\\
%          \hline
%          Average degree & 1.87\\
%          \hline
%          Density of graph & 0.000171\\
%          \hline
%          Number of connected components & 1368\\
%          \hline
%          Nodes in LCC & 6839\\
%          \hline
%          Edges in LCC & 7481\\
%          \hline
    
%     \end{tabular}
%     \caption{Statistics of the graph created from OMIM.}
%     \label{tab:omim_dataset}
% \end{table}





\cut{
%\hadi{Introduce the {\bf G}ene, {\bf D}isease, {\bf P}henotype {\bf R}elation (GDPR) dataset -- need to include phenotypes as well.}

\begin{table}[t]\small
    \centering
    \begin{tabular}{|l|l|}\hline  
       {\bf Metric} & {\bf Value} \\\hline 
         \# Gene nodes &  4,274\\\hline
         \# Disease nodes & 6,143\\\hline
         \# Disease type nodes & 472\\\hline
         \# Phenotype nodes & 9,603\\\hline
         \# Nodes in LCC & 20,264 \\\hline
         \# Edges & 964,222 \\\hline
             \hspace{5pt} $\rightarrow$ Gene-Disease & 6,284 \\\hline
             \hspace{5pt} $\rightarrow$ Gene-Phenotype & 595,296 \\\hline
             \hspace{5pt} $\rightarrow$ Disease-Disease type & 3,912 \\\hline
             \hspace{5pt} $\rightarrow$ Disease-Phenotype & 358,730 \\\hline
         \# Edges in LCC & 964,087 \\\hline
         \# Connected components & 94 \\\hline
         Average node degree & 94.11 \\\hline
             \hspace{5pt} $\rightarrow$ Genes & 140.75 \\\hline
             \hspace{5pt} $\rightarrow$ Diseases & 60.04 \\\hline
             \hspace{5pt} $\rightarrow$ Disease types & 8.28 \\\hline
             \hspace{5pt} $\rightarrow$ Phenotypes & 99.35 \\\hline
         Graph density & 0.004592 \\\hline
    \end{tabular}
    \caption{Statistics of GDPR dataset.}
    %\hadi{please add if you have time, otherwise remove.}
    %\hadi{please add missing values.}
    \label{tab:omim_dataset}
\end{table}


The Online Mendelian Inheritance in Man, OMIM,~\cite{amberger2019omim} dataset is the primary repository of curated information on genes, rare diseases and their causal relations. Each gene and disease is provided with a detailed textual summary based on expert reviews of the relevant biomedical literature.\footnote{An example of a textual summary for LEUKEMIA can be found at  https://omim.org/entry/608232}. 
There exist three categories of information in OMIM: genes, diseases, and diseases types. 
Genes are basic units of heredity and sequences of nucleotides in DNA or RNA. 
Disease types are collections of similar diseases across the same genome. 
% There are more than 16000 genes, 7000 diseases and 505 disease type in OMIM.
Genes or diseases may link to one or more diseases or genes respectively. 
%and vice-versa . 
Similarly, a disease can be associated with one or more disease types.
Each verified relation between genes and diseases contains references to scientific literature providing evidence about the corresponding relation.
%
In addition, OMIM provides detailed textual summaries for genes and diseases describing their clinical characteristics. The textual summary of a gene contains a short description about the gene, its functions, cloning information and gene structure. The textual summary of a disease contains a short description, clinical features, inheritance and its history. There are many genes and diseases in this dataset which are not associated to any disease or genes. As a pre-processing step, we remove genes/diseases that are not linked to any disease/gene respectively. 

\todo[inline]{explanation to add: relevant information present in the textual summary and why not to include publication}
%OMIM is a challenging dataset, as the data is sparse with nearly half of the edges does not corresponds to gene-phenotype pairs. Moreover, the network contains fewer edges than nodes indicating there are several disconnected components. Such disconnected components does not allow graph neural networks to propagate information and hinder learning the graph structure. 


% \subsection{Network Construction}
% \label{NetConst}
% Using genes, phenotypes, diseases and disease series we constructed the graph using the relations provided by the OMIM dataset. After mapping relations to the graph, total number of nodes in the graph were $10899$ and the total number of edges in the graph were $10196$ which results in sparse graph and the graph contains several disconnected components. This is due to the type and nature of relations between the gene-phenotypes/diseases pairs. Such disconnected components and sparsity in the graph makes the learning task challenging as it  does not allow graph neural networks to propagate information and hinder in learning the graph structure. To overcome this problem, 


% \nidhi{Human Phenotype Ontology (HPO) provides standard vocabulary to describe abnormalities encountered in human diseases. Each phenotype present in the HPO have a textual summary describing the characteristics of the phenotype. In order to keep the dataset medically consistent, we associated gene and diseases present in the OMIM dataset with corresponding phenotypes from HPO. To obtain those associations, we used HPO  relation file provided by \cite{HPO}. 
 
%  In contrast to HPO, OMIM focuses on rare diseases and each gene on an average is associated with at most 2 diseases creating sparsity issues. We consider only gene-disease from OMIM in which there is atleast one gene associated with at least one disease and vice-versa. Combining HPO helps to alleviate the sparsity issue and create a stand-alone dataset to study about rare diseases. Resulting dataset contains information about gene, diseases, diseases type and phenotypes. 
% %To study the causality between genes and diseases, from the OMIM dataset we have used only those genes and diseases which have at least one phenotype or gene. Table \ref{tab:omim_dataset} shows the statistics of the graph. As evident from average degree and density of the graph in Table \ref{tab:omim_dataset},  the network generated from OMIM is sparse. This is because each genes is on an average connected to at most 2 diseases as the diseases are rare.
%  %Such a process helps to make the graph dense and connect several disconnected components. Resulting graph contains four categories of nodes -- genes, diseases, disease types, and phenotypes.
%  }
 

Human Phenotype Ontology, HPO,~\cite{hpo} provides standard vocabulary to describe abnormalities encountered in human diseases. Each phenotype in HPO has a textual summary describing the clinical characteristics of the phenotype. HPO provides mapping of its phenotypes to gene and diseases in the OMIM dataset. We use this mapping to compile the {\bf G}ene, {\bf D}isease, {\bf P}henotype {\bf R}elation (GDPR) dataset, which contains relations between genes, diseases, disease types and phenotypes. 

Table~\ref{tab:omim_dataset} provides graph-level statistics of GDPR.\footnote{We note that, since OMIM focuses on rare diseases, each gene is linked to at most two diseases, leading to sparsity issues at gene-disease level. HPO helps alleviate this sparsity issue through phenotype nodes linked to genes and diseases.}  

% Resulting dataset contains information about gene, diseases, diseases type and phenotypes. 




% \begin{table}[]
%     \centering
%     \begin{tabular}{|p{4cm}|l|}
%         \hline
%          \# of Genes &  4274\\
%          \hline
%          Number of Disease Series & 472\\
%          \hline
%          Number of Disease & 6143\\
%          \hline
%          Number of Total Nodes & 10889\\
%          \hline
%          Number of edges & 10196\\
%          \hline
%          Average degree & 1.87\\
%          \hline
%          Density of graph & 0.000171\\
%          \hline
%          Number of connected components & 1368\\
%          \hline
%          Nodes in LCC & 6839\\
%          \hline
%          Edges in LCC & 7481\\
%          \hline
    
%     \end{tabular}
%     \caption{Statistics of the graph created from OMIM.}
%     \label{tab:omim_dataset}
% \end{table}

}

==> sections/supplementry.tex <==
\setcounter{figure}{0}    
\section{In-domain embeddings improves the  performance}

For these experiments, we re-train our model without additional textual feature but with different embedding initialization. As shown in Figure \ref{fig:ablation_w_feature} and \ref{fig:ablation_wo_feature}, Doc2Vec embeddings result in an overall better performance than BioBERT and random initialization approaches across the datasets. We attribute this result to in-domain training using text summaries of genes, diseases and phenotypes associated to rare diseases. In addition, the performance using BioBERT embeddings is considerably lower than that of other embeddings including Random. This is perhaps due to pre-training of BioBERT using a large scale PubMED dataset, which has a significantly lower prevalence of publications on rare vs. common diseases. On the other hand, we directly optimize Doc2Vec on in the domain datasets, which leads to higher performance of the model. We tried to fine tune BioBERT on our corpus but as the textual summaries were long, only few initial sentences were considered rest were discarded. Hence we focus on fine tuning Doc2Vec. 

\section{Additional Features improves the performance}

For these experiments, we re-train our models and include additional feature (i.e., relevance scores for \gdpr~and sentence embeddings for \pgr), with different node embedding initialization. 
Figure \ref{fig:ablation_w_feature} show that additional features improve the F1-scores of our model across all datasets and embedding initialization. 
These results show that both textual features and information obtained from graph structure contribute to predicting relations between nodes. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.42]{images/ablation_w_feature.pdf}
    \caption{Performance of \gtnn{}  with Trend-SL with additional features.}
    \label{fig:ablation_w_feature}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.42]{images/ablation_wo_feature.pdf}
    \caption{Performance of \gtnn{}  with Trend-SL without additional features.}
    \label{fig:ablation_wo_feature}
\end{figure}

\section{Inversions occur with falling or rising loss trends}
\begin{figure*}[!t]
    \centering
    \subfigure{\includegraphics[scale=0.45]{images/easy_fraction_analysis_1d 3.pdf}\label{fig:e2h_fraction_1d}}
    \subfigure{\includegraphics[scale=0.45]{images/hard_fraction_analysis_1d 2.pdf}\label{fig:h2e_fraction_1d}}
    \caption{Inversion heatmap of the examples when easy example converts to hard example (left) and vice versa (right)}
    \label{fig:fraction1d}
\end{figure*} 
Fig \ref{fig:fraction1d} shows the inversion heatmap for Easy-to-Hard and Hard-to-Easy for consecutive epoch where the y-axis fraction indicates the number of examples that were considered easy at epoch $e$ and had a rising trend which were converted into hard examples at epoch $e+1$. Similarly for Hard-to-Easy inversion heatmap. In Hard-to-Easy inversion the examples were hard at current epoch but had falling trend to eventually be inverted to easy examples. The area under the curve for Easy-to-Hard with rising trend is 24.87 and 4.51 for Hard-to-Easy. 

